CANDiS: Coupled & Attention-Driven Neural Distant Supervision

Distant Supervision for Relation Extraction uses heuristically aligned text data with an existing knowledge base as training data. The unsupervised nature of this technique allows it to scale to web-scale relation extraction tasks, at the expense of noise in the training data. Previous work has explored relationships among instances of the same entity-pair to reduce this noise, but relationships among instances across entity-pairs have not been fully exploited. We explore the use of inter-instance couplings based on verb-phrase and entity type similarities. We propose a novel technique, CANDiS, which casts distant supervision using inter-instance coupling into an end-to-end neural network model. CANDiS incorporates an attention module at the instance-level to model the multi-instance nature of this problem. CANDiS outperforms existing state-of-the-art techniques on a standard benchmark dataset.

==> sections/conclusion.tex <==
\section{Conclusion}

In this paper, we present \system{} for robust distant supervision. As we have shown, incorporating inter-instance coupling information into the the representations significantly boosts performance over a broad recall range in the relation extraction task. It would be infomative to see how this sort of coupling affects representation learning for other tasks. As future work we would like to explore more sophisticated forms of couplings, and richer embedding models.  

==> sections/related_work.tex <==
\section{Related Work}



Distant supervision for Relation Extraction was introduced by \cite{mintz:2009} using a Freebase-aligned Wikipedia corpus. A large proportion of the subsequent work in this field has aimed to relax the strong assumptions that the original DS model made. \cite{riedel:2010} introduced the \textit{expressed-at-least-once} assumption in a factor graph model as an aggregating mechanism over mention level predictions. Work by \cite{hoffmann:2011} \cite{ritter:2013} \cite{surdeanu:2012} are crucial increments to \cite{riedel:2010} to improve RE further. \cite{zeng:2015} proposed a Piecewise Convolutional Neural Network (PCNN) to tackle the issue of hand-crafted feature engineering. 

A few papers propose the addition of background knowledge to reduce noise in training data. \cite{weston:2013} proposes a joint-embedding model for text and KB entities where the known part of the KB is utilized as part of the supervision signal. \cite{han:2016} use indirect supervision like consistency between relation labels, consistency between relations and arguments and consistency between neighbour instances using Markov logic networks. This work is similar to our approach, however, we use different coupling factors on a sentence level, in a neural network based multitask framework.

\cite{zheng:2016} aimed to leverage \textit{inter-sentence} information for relation extraction in a ranking model. The hypothesis explored is that for a particular entity-pair, each mention alone may not be expressive enough of the relation in question, but information from several mentions may be required to decisively make a prediction. In our memory-network component, this aggregation is explored in more detail and with interpretable results.
% TODO: add multi task and siamese network references if space remains


